Pinning Down the Strong Wilber 1 Bound for Binary Search Trees

The dynamic optimality conjecture, postulating the existence of an $O(1)$-competitive online algorithm for binary search trees (BSTs), is among the most fundamental open problems in dynamic data structures. Despite extensive work and some notable progress, including, for example, the Tango Trees (Demaine et al., FOCS 2004), that give the best currently known $O(\log \log n)$-competitive algorithm, the conjecture remains widely open. One of the main hurdles towards settling the conjecture is that we currently do not have approximation algorithms achieving better than an $O(\log \log n)$-approximation, even in the offline setting. All known non-trivial algorithms for BST's so far rely on comparing the algorithm's cost with the so-called Wilber's first bound (WB-1). Therefore, establishing the worst-case relationship between this bound and the optimal solution cost appears crucial for further progress, and it is an interesting open question in its own right. Our contribution is two-fold. First, we show that the gap between the WB-1 bound and the optimal solution value can be as large as $\Omega(\log \log n/ \log \log \log n)$; in fact, the gap holds even for several stronger variants of the bound. Second, we provide a simple algorithm, that, given an integer $D>0$, obtains an $O(D)$-approximation in time $\exp\left(O\left (n^{1/2^{\Omega(D)}}\log n\right )\right )$. In particular, this gives a constant-factor approximation sub-exponential time algorithm. Moreover, we obtain a simpler and cleaner efficient $O(\log \log n)$-approximation algorithm that can be used in an online setting. Finally, we suggest a new bound, that we call {\em Guillotine Bound}, that is stronger than WB, while maintaining its algorithm-friendly nature, that we hope will lead to better algorithms. All our results use the geometric interpretation of the problem, leading to cleaner and simpler analysis.

==> semi-to-permutation.tex <==

\section{Upper Bound for $\WB(X^*)$}

In this section we show that $\WB(X^*)=O(N^*\log\log\log N^*)$.

In fact we prove a stronger theorem that allows us to transform any semi-permutation $X$ into a permutation $X'$, without increasing the cost of the Wilber Bound by much.

\begin{theorem}\label{thm: semi to permutation}
	Let $X$ be a semi-permutation, and let $\cset$ be the set of all active columns for $X$. Assume that every column of $\cset$ contains at most $q$ points of $X$. Let $X'$ be a new instance, obtained from $X$, by replacing every column $C\in \cset$ with a collection $\bset(C)$ of $q$ columns, and placing all points of $X\cap C$ on the columns of $\bset(C)$, so that they form a monotonically increasing sequence, while preserving their rows. Then $\WB(X')\leq 4\WB(X)+O(|\cset|\cdot q)$.
\end{theorem}

Assume that Theorem \ref{thm: semi to permutation} is correct. Notice that $X^*$ is obtained from $\hat X$ using the same transformation as the one in the theorem statement, with $q=\log N$ and $|\cset|=N$. Therefore, $\WB(X^*)\leq 4\WB(\hat X)+O(N\log N)=O(N^*\log\log\log N^*)$, since $N^*=N\log N$. The remainder of this section is dedicated to the proof of Theorem \ref{thm: semi to permutation}.

For the sake of the proof, it would be convenient for us to define a more general notion of the Wilber Bound.


\paragraph{Extension of Wilber Bound to Forbidden Points.}
Assume that we are given any set $\tX$ of input points that is a semi-permutation, and let $\tlset$ be the set of all vertical lines with half-integral coordinates.

Assume further that we are given a collection $F\subseteq \tX$ of points, that we refer to as \emph{forbidden points}. We now define a new Wilber Bound with respect to the forbidden points, $\WB^F(\tX)$.

Consider any permutation $\tsigma$ of the lines in $\tlset$, and let $T=T(\tsigma)$ be the partitioning tree associated with $\tsigma$. Consider some vertex $v\in V(T)$; let $S=S(v)$ be the vertical strip associated with $v$, and let $L\in \tlset$ be the vertical line that belongs to $v$. We let $\cro_{\tsigma}(L)$ be the set of all crossings $(p,p')$ that contribute to $\cost(L)$; that is, $p$ and $p'$ are two points that lie in $S$ on two opposite sides of $L$, and no other point of $\tX\cap S$ lies between the row of $p$ and the row of $p'$. Let $\cro_{\tsigma}=\bigcup_{L\in \tlset}\cro_{\tsigma}(L)$, so $|\cro_{\tsigma}|=\WB_{\tsigma}(X)$.

In order to define the modified Wilber Bound, consider again some vertex $v\in V(T)$, the line $L$ that belongs to it, and the set $\cro_{\tsigma}(L)$ of crossings that we have defined for it. We say that a crossing $(p,p')\in \cro_{\tsigma}(L)$ is \emph{forbidden} iff at least one of $p,p'$ lie in $F$; otherwise the crossing is \emph{allowed}. We let $\cro^F_{\tsigma}(L)$ be the set of crossings obtained from $\cro_{\tsigma}(L)$ by discarding all forbidden crossings from it. We then let $\cro^F_{\tsigma}=\bigcup_{L\in \tlset}\cro^F_{\tsigma}(L)$, and $\WB^F_{\tsigma}(\tX)=|\cro^F_{\tsigma}|$. Finally, we let $\WB^F(\tX)$ be the maximum, over all permutations $\tsigma$ of the lines of $\tlset$, of $\WB^F_{\tsigma}(\tX)$.

We emphasize that $\WB^F(\tX)$ is not necessarily the same as $\WB(\tX\setminus F)$, as some crossings of the instance $\tX\setminus F$ may not correspond to allowed crossings of instance $\tX$.


\paragraph{Proof Overview and Notation.}

We assume that we are given a set $X$ of input points, that is a semi-permutation. We denote the set of active columns by $\cset=\set{C_1,\ldots,C_N}$, where the columns are indexed in their natural left-to-right order. For convenience, we denote by $X_i\subseteq X$ the set of points lying on the column $C_i$. Recall that for all $1\leq i\leq N$, $|C_i|\leq q$. %

Recall that $X'$ is an instance, obtained from $X$, by replacing every column $C_i\in \cset$ with a collection $\bset(C_i)$ of $q$ columns, and placing all points of $X_i$ on the columns of $\bset(C_i)$, so that they form a monotonically increasing sequence, while preserving their rows. We denote the set of points of $X'$ lying on the columns of $\bset(C_i)$ by $X'_i$.


It would be convenient for us to slightly modify the instance $X$ by simply multiplying all $x$-coordinates of points of $X$ and of columns of $\cset$ by factor $2$. Note that this does not affect the value of the optimal solution or of the Wilber Bound; but it ensures that every consecutive pair of columns in $\cset$ is separated by a column with an integral $x$-coordinate. We let $\lset$ be the set of all vertical lines with half-integral coordinates in the resulting instance $X$.

Similarly, we modify the instance $X'$, by inserting, for every consecutive pair $C_i,C_{i+1}$ of columns of $\cset$, a new column with an integral coordinate that lies between the columns of $\bset(C_i)$ and the columns of $\bset(C_{i+1})$. This transformation does not affect the optimal solution cost or the value of the Wilber Bound. We denote by $\lset'$ the set of all vertical lines with half-integral coordinates, in the resulting instance $X'$.

Consider any column $C_i\in \cset$. We denote by $\lset'(C_i)=\set{L_i^1,\ldots,L_i^{q+1}}$ the set of $q+1$ consecutive vertical lines in $\lset'$, where $L_i^1$ appears immediately before the first column of $\bset(C_i)$, and $L_i^{q+1}$ appears immediately after the last column of $\bset(C_i)$. Notice that $\lset'=\bigcup_{C_i\in \cset}\lset'(C_i)$.

Recall that our goal is to show that $\WB(X')\leq 4\WB(X)+O(|\cset|\cdot q)$. In order to do so, we fix a permutation $\sigma'$ of $\lset'$ that maximizes $\WB_{\sigma'}(X')$, so that $\WB(X')=\WB_{\sigma'}(X')$. We then gradually transform it into a permutation $\sigma$ of $\lset$, such that $\WB_{\sigma}(X)\geq \WB_{\sigma'}(X')/4-O(|\cset|\cdot q)$. This will prove that $\WB(X)\geq \WB_{\sigma}(X)\geq \WB_{\sigma'}(X')/4-O(|\cset|\cdot q)=\WB(X')/4-O(Nq)$.

In order to perform this transformation, we will process every column $C_i\in \cset$ one-by-one. When column $C_i$ is processed, we will ``consolidate'' all lines of $\lset'(C_i)$, so that they will appear almost consecutively in the permutation $\sigma'$, and we will show that this process does not increase the Wilber Bound by too much. The final permutation that we obtain after processing every column in $\cset$ can then be naturally transformed into a permutation $\sigma$ of $\lset$, whose Wilber Bound cost is similar. The main challenge is to analyze the increase in the Wilber Bound in every iteration. In order to facilitate the analysis, we will work with the extended Wilber Bound. Specifically, we will define a set $F\subseteq X'$ of forbidden points, such that $\WB_{\sigma'}^F(X')\geq \WB_{\sigma'}(X')/4$. For every column $C\in \cset_i$, we will also define a bit $b(C)\in \set{0,1}$, that will eventually guide the way in which the lines of $\lset'(C)$ are consolidated. As the algorithm progresses, we will modify the set $F$ of forbidden points by discarding some points from it, and we will show that the increase in the Wilber Bound with respect to the new set $F$ is small relatively to the original Wilber Bound with respect to the old set $F$. We start by defining the set $F$ of forbidden points, and the bits $b(C)$ for the columns $C\in \cset$. We then show how to use these bits in order to transform permutation $\sigma'$ of $\lset'$ into a new permutation $\sigma''$ of $\lset'$, which will in turn be transformed into a permutation $\sigma$ of $\lset$.

From now on we assume that the permutation $\sigma'$ of the lines in $\lset'$ is fixed.

\paragraph{Defining the Set $F$ of Forbidden Points.}
Consider any column $C_i\in \cset$. We denote by $L^*_i\in \lset'_i$ the vertical line that appears first in the permutation $\sigma'$ among all lines of $\lset'_i$, and we denote by $L^{**}_i$ the line that appears last in $\sigma'$ among all lines of $\lset'_i$. 

We perform $N$ iteration. In iteration $i$, for $1\leq i\leq N$, we consider the column $C_i$. We let $b_i\in \set{0,1}$ be a random bit chosen uniformly at random, independently from all other random bits. If $b_i=0$, then all points of $X'_i$ that lie to the left of $L^*_i$ are added to the set $F$ of forbidden points; otherwise, all points of $X'_i$ that lie to the right of $L^*_i$ are added to the set $F$ of forbidden points.

Note that, if we let $(p,p')\in \cro_{\sigma'}$ be any crossing, then with probability at least $1/4$, this crossing remains allowed. Therefore, the expectation of $|\cro^F_{\sigma'}|$ is at least $|\cro_{\sigma'}|/4$. So there is a choice of the bits in $\set{b(C_i)}_{C_i\in \cset}$, such that, if we define the set $F$ of forbidden points with respect to these bits as before, then $|\cro^F_{\sigma'}|\geq |\cro_{\sigma'}|/4$. From now on we assume that the values of the bits in $\set{b(C_i)}_{C_i\in \cset}$ are fixed, and that the resulting set $F$ of forbidden points satisfies that $|\cro^F_{\sigma'}|\geq |\cro_{\sigma'}|/4$.

\paragraph{Transforming $\sigma'$ into $\sigma''$.}
We now show how to transform the original permutation $\sigma'$ of $\lset'$ into a new permutation $\sigma''$ of $\lset'$, which we will later transform into a permutation $\sigma$ of $\lset$. We perform $N$ iterations. The input to the $i$th iteration is a permutation $\sigma_i$ of $\lset'$ and a subset $F_i\subseteq F$ of forbidden points. The output of the iteration is a new permutation $\sigma_{i+1}$ of $\lset'$, and a set $F_{i+1}\subseteq F_i$ of forbidden points. The final permutation is $\sigma''=\sigma_{N+1}$, and the final set $F_{N+1}$ of forbidden points will be empty. The input to the first iteration is $\sigma_1=\sigma'$ and $F_1=F$. We now fix some $1\leq i\leq N$, and show how to execute the $i$th iteration. Intuitively, in the $i$th iteration, we consolidate the lines of $\lset'_i$. Recall that we have denote by $L^*_i,L^{**}_i\in \lset'_i$ the first and the last line of $\lset'_i$ in the permutation $\sigma'$. We only move the lines of $\lset'_i$ in iteration $i$, so this ensures that, in permutation $\sigma_i$, the first line of $\lset'_i$ that appears in the permutation is $L^*_i$, and the last line is $L^{**}_i$.

We now describe the $i$th iteration. Recall that we are given as input a permutation $\sigma_i$ of the lines of $\lset'$, and a subset $F_i\subseteq F$ of forbidden points. 
We consider the column $C_i\in \cset$ and the corresponding bit $b(C_i)$.

Assume first that $b(C_i)=0$; recall that in this case, all points of $X'$ that lie on the columns of $\bset(C_i)$ to the left of $L^*_i$ are forbidden.  We start by switching the locations of $L^*_i$ and $L^1_i$ in the permutation $\sigma_i$ (recall that $L^1_i$ is the leftmost line in $\lset'_i$). Therefore, $L^1_i$ becomes the first line of $\lset'_i$ in the resulting permutation. Next, we
consider the location of line $L^{**}$ in the resulting permutation, and we replace this line with the lines $L_i^{q+1},L_i^2,L_i^3,\ldots,L_i^{q}$ in this order. This defines the new permutation $\sigma_{i+1}$.

Assume now that $b(C_i)=1$;  recall that in this case, all points of $X'$ that lie on the columns of $\bset(C_i)$ to the right of $L^*_i$ are forbidden.   We start by switching the locations of $L^*_i$ and $L_i^{q+1}$ in the permutation $\sigma_i$ (recall that $L_i^{q+1}$ is the rightmost line in $\lset'_i$). Therefore, $L_i^{q+1}$ becomes the first line of $\lset'_i$ in the resulting permutation. Next, we
consider the location of line $L^{**}$ in the resulting permutation, and we replace this line with the lines $L_i^1,L_i^2,L_i^3,\ldots,L_i^q$ in this order. This defines the new permutation $\sigma_{i+1}$.

Lastly, we discard from $F_i$ all points that lie on the columns of $\bset(C_i)$, obtaining the new set $F_{i+1}$ of forbidden points.

Once every column of $\cset$ is processed, we obtain a final permutation $\sigma_{N+1}$ that we denote by $\sigma''$, and the final set $F_{N+1}=\emptyset$ of forbidden lines. The following lemma is central to our analysis. It shows that the Wilber Bound does not decrease by much after every iteration. The Wilber Bound is defined with respect to the appropriate sets of forbidden points.


\begin{lemma}\label{lemma: small change}
	For all $C_i\in \cset$,  $\WB^{F_{i+1}}_{\sigma_{i+1}}(X')\geq \WB^{F_i}_{\sigma_i}(X')-O(q)$.
\end{lemma}

Assume first that the lemma is correct. Recall that we have ensured that $\WB^{F_1}_{\sigma_1}(X')=\WB^F_{\sigma'}(X')\geq \WB_{\sigma'}(X')/4$. Since $F_{N+1}=\emptyset$, this will ensure that $\WB_{\sigma''}(X')\geq \WB^F_{\sigma'}(X')-O(Nq)\geq \WB_{\sigma'}(X')/4-O(Nq)$. We now focus on the proof of the lemma.


\begin{proof}
	In order to simplify the notation, we denote $\sigma_i$ by $\tsigma$, $\sigma_{i+1}$ by $\tsigma'$, $F_i$ by $\tF$, and $F_{i+1}$ by $\tF'$.
	
	
	Consider a line $L\in \lset'$. Recall that $\cro_{\tsigma}(L)$ is the set of all crossings that are charged to the line $L$ in permutation $\tsigma$. Recall that $\cro^{\tF}_{\tsigma}(L)\subseteq \cro_{\tsigma}(L)$ is obtained from the set  $\cro_{\tsigma}(L)$ of crossings, by discarding all crossings $(p,p')$ where $p\in \tF$ or $p'\in \tF$ holds. The set $\cro^{\tF'}_{\tsigma'}(L)$ of crossings is defined similarly.
	
	We start by showing that for every line $L\in \lset'$ that does not lie in $\lset'_i$, the number of crossings charged to it does not decrease, that is, $\cro^{\tF'}_{\tsigma'}(L)\geq\cro^{\tF}_{\tsigma}(L)$.
	
	\begin{claim}\label{claim: lines outside of block do not change}
		For every line $L\in \lset'\setminus \lset'_i$, $\cro^{\tF'}_{\tsigma'}(L)\geq\cro^{\tF}_{\tsigma}(L)$.
	\end{claim}
	\begin{proof}
		Consider any line $L\in \lset'\setminus \lset(C)$. Let $v\in V(T_{\tsigma})$ be the vertex to which $L$ belongs, and let $S=S(v)$ be the corresponding strip. Similarly, we define $v'\in V(T_{\tsigma'})$ and $S'=S(v')$ with respect to $\tsigma'$.  
		Recall that $L^*_i$ is the first line of $\lset'_i$ to appear in permutation in $\sigma'$, and $L^{**}_i$ is the last such line. We now consider five cases.
		
		
	\paragraph{Case 1.}	The first case happens if $L$ appears before line $L^*_i$ in the permutation $\tsigma$. Notice that the prefixes of the permutations $\tsigma$ and $\tsigma'$ are identical up to the location in which $L^*_i$ appears in $\tsigma$. Therefore, $S=S'$, and $\cro_{\tsigma}(L)=\cro_{\tsigma'}(L)$. Since $\tF'\subseteq \tF$, every crossing that is forbidden in $\tsigma'$ was also forbidden in $\tsigma$. So $\cro_{\tsigma}^{\tF}(L)\subseteq \cro_{\tsigma'}^{\tF'}(L)$, and $\cro^{\tF'}_{\tsigma'}(L)\geq\cro^{\tF}_{\tsigma}(L)$.
		
	\paragraph{Case 2.} The second case happens if $L$ appears after $L^{**}_i$ in $\tsigma$. Notice that, if we denote by $\tilde \lset\subseteq \lset'$ the set of all lines of $\lset'$ that lie before $L$ in $\tsigma$, and define $\tilde \lset'$ similarly for $\tsigma'$, then $\tilde \lset=\tilde \lset'$. Therefore, $S=S'$ holds. Using the same reasoning as in Case 1,  $\cro^{\tF'}_{\tsigma'}(L)\geq\cro^{\tF}_{\tsigma}(L)$.
	
	\paragraph{Case 3.}
The third case is when $L$ appears between $L^*_i$ and $L^{**}_i$ in $\tsigma$, but neither boundary of the strip $S$ belongs to $\lset'_i$. If we denote by $\tilde \lset\subseteq \lset'\setminus \lset'_i$ the set of all lines of $\lset'\setminus\lset'_i$ that lie before $L$ in $\tsigma$, and define $\tilde \lset'\setminus\lset'_i$ similarly for $\tsigma'$, then $\tilde \lset=\tilde \lset'$. Therefore, $S=S'$ holds. Using the same reasoning as in Cases 1 and 2,  $\cro^{\tF'}_{\tsigma'}(L)\geq\cro^{\tF}_{\tsigma}(L)$.

\paragraph{Case 4.}
		The fourth case is when $L$  appears between $L^*$ and $L^{**}$ in the permutation $\tsigma$, and the left boundary of $S$ belongs to $\lset'_i$. Notice that the left boundary of $S$ must either coincide with $L^*$, or appear to the right of it.
		
		Assume first that $b(C_i)=0$, so we have replaced $L^*_i$ with the line $L_i^1$, that lies to the left of $L^*(C)$. Since no other lines of $\lset'_i$ appear in $\tsigma'$ until the original location of line $L^{**}_i$, it is easy to verify that the right boundary of $S'$ is the same as the right boundary of $S$, and its left boundary is the line $L_i^1$, that is, we have pushed the left boundary to the left. %
		In order to prove that
		 $|\cro^{\tF'}_{\tsigma'}(L)|\geq|\cro^{\tF}_{\tsigma}(L)|$, we map every crossing $(p_1,p_2)\in \cro^{\tF}_{\tsigma}(L)$ to some crossing $(p_1',p_2')\in \cro^{\tF'}_{\tsigma'}(L)$, so that no two crossings of $\cro^{\tF}_{\tsigma}(L)$ are mapped to the same crossing of $\cro^{\tF'}_{\tsigma'}(L)$.
		 %
		 
		 Consider any crossing $(p_1,p_2)\in \cro^{\tF}_{\tsigma}(L)$. We know that $p_1,p_2\in S$, and they lie on opposite sides of $L$. We assume w.l.o.g. that $p_1$ lies to the left of $L$. %
 		 Moreover, no point of $X'\cap S$ lies between the row of $p_1$ and the row of $p_2$. 
		 It is however possible that $(p_1,p_2)$ is not a crossing of $\cro_{\tsigma'}(L)$, since by moving the left boundary of $S$ to the left, we add more points to the strip, some of which may lie between the row of $p_1$ and the row of $p_2$. Let $A$ be the set of all points that lie between the row of $p_1$ and the row of $p_2$ in $S'$. Notice that the points of $A$ must lie between the lines $L^*$ and $L_i^1$, so they are forbidden in $\tF$, but not in $\tF'$. Let $a\in A$ be the point of $a$ whose row is closest to the row of $p_2$; if $A=\emptyset$, then we set $a=p_1$. Then $(a,p_2)$ define a crossing in $\cro_{\tsigma'}(L)$, and, since neither point lies in $\tF'$, $(a,p_2)\in \cro^{\tF'}_{\tsigma'}(L)$. In this way, we map we map every crossing $(p_1,p_2)\in \cro^{\tF}_{\tsigma}(L)$ to some crossing $(p_1',p_2')\in \cro^{\tF'}_{\tsigma'}(L)$. It is easy to verify that no two crossings of $\cro^{\tF}_{\tsigma}(L)$ are mapped to the same crossing of $\cro^{\tF'}_{\tsigma'}(L)$. We conclude that $|\cro^{\tF'}_{\tsigma'}(L)|\geq|\cro^{\tF}_{\tsigma}(L)|$.
		 
		 
		 
		
		Lastly, assume that $b(C)=1$. Recall that the set of all points of $X'$ lying between $L^*_i$ and $L_{i}^{q+1}$ is forbidden in $\tF$ but not in $\tF'$, and that we have replaced $L^*_i$ with the line $L_i^{q+1}$, that lies to the right of $L^*_i$. Therefore, the right boundary of $S$ remains the same, and the left boundary is pushed to the right. %
		 In order to prove that
		$|\cro^{\tF'}_{\tsigma'}(L)|\geq|\cro^{\tF}_{\tsigma}(L)|$, we show that every crossing $(p_1,p_2)\in \cro^{\tF}_{\tsigma}(L)$ belongs to $\cro^{\tF'}_{\tsigma'}(L)$. Indeed, consider any crossing $(p_1,p_2)\in \cro^{\tF}_{\tsigma}(L)$. We know that $p_1,p_2\in S$, and they lie on opposite sides of $L$. We assume w.l.o.g. that $p_1$ lies to the left of $L$. Since $p_1$ cannot be a forbidden point, it must lie to the right of $L_i^{q+1}$. Moreover, no point of $X\cap S$ lies between the row of $p_1$ and the row of $p_2$. It is now easy to verify that $(p_1,p_2)$ is also a crossing in $\cro^{\tF'}_{\tsigma'}(L)$.
		
		\paragraph{Case 5.}
		The fifth case happens when $L$ appears between $L^*_i$ and $L^{**}_i$ in the permutation $\tsigma$, and the right boundary of $S$ belongs to $\lset_i'$. This case is symmetric to the fourth case and is analyzed similarly.
	\end{proof}
	
	It now remains to analyze the crossings of the lines in $\lset'_i$. We do so in the following two claims. The first claim shows that switching $L^*_i$ with $L^1_i$ or $L^{q+1}_i$ does not decrease the number of crossings.
	
	\begin{claim}
		If $b=0$, then	$|\cro^{\tF'}_{\tsigma'}(L_i^1)|\geq |\cro^{\tF}_{\tsigma}(L^*_i)|$; if $b=1$, then $|\cro^{\tF'}_{\tsigma'}(L_i^{q+1})|\geq |\cro^{\tF}_{\tsigma}(L^*_i)|$.
	\end{claim}
	
	\begin{proof}
		Assume first that $b=0$, so we have replaced $L^*_i$ with $L_i^1$ in the permutation. As before, we let $v\in V(T_{\tsigma})$ be the vertex to which $L^*_i$ belongs, and we let $S=S(v)$ be the corresponding strip. Similarly, we define $v'\in V(T_{\tsigma'})$ and $S'=S(v')$ with respect to line $L_i^1$ and permutation $\tsigma'$. Notice that, until the appearance of $L^*_i$ in $\tsigma$, the two permutations are identical. Therefore, $S=S'$ must hold. Recall also that all points of $X'$ that lie between $L^*_i$ and $L_i^1$ are forbidden in $\tF$, but not in $\tF'$. In order to show that $|\cro^{\tF'}_{\tsigma'}(L_i^1)|\geq |\cro^{\tF}_{\tsigma}(L^*_i)|$, it is enough to show that every crossing $(p_1,p_2)\in \cro^{\tF}_{\tsigma}(L^*_i)$ also lies in $\cro^{\tF'}_{\tsigma'}(L_i^1)$. 
		
		Consider now some crossing $(p_1,p_2)\in \cro^{\tF}_{\tsigma}(L^*_i)$. Recall that one of $p_1,p_2$ must lie to the left of $L_i^*$ and the other to the right of it, with both points lying in $S$. Assume w.l.o.g. that $p_1$ lies to the left of $L_i^*$. Since $p_1\not\in \tF$, it must lie to the left of $L^1_i$. Moreover, no point of $X'\cap S$ may lie between the row of $p_1$ and the row of $p_2$. It is then easy to verify that $(p_1,p_2)$ is also a crossing in $\cro^{\tF'}_{\tsigma'}(L_i^1)$, and so $|\cro^{\tF'}_{\tsigma'}(L_i^1)|\geq |\cro^{\tF}_{\tsigma}(L^*_i)|$.
		
		The second case, when $b=1$, is symmetric.
	\end{proof}

Lastly, we show that for all lines $L\in \lset'_i\setminus\set{L_i^*}$, their total contribution to $\cro^{\tF}_{\tsigma}$ is small, in the following claim.

\begin{claim}\label{claim: lines in li contribute little}
	$\sum_{L\in \lset_i'\setminus\set{L_i^*}}|\cro^{\tF}_{\tsigma}(L)|\leq O(q)$.
\end{claim}

Assume first that the claim is correct. We have shown so far that the total contribution of all lines in $\lset_i'\setminus\set{L_i^*}$ to $\cro^{\tF}_{\tsigma}$ is $O(q)$; that the contribution of one of the lines $L_i^1,L_i^{q+1}$ to $\cro^{\tF'}_{\tsigma'}$ is at least as large as the contribution of $L_i^*$ to $\cro^{\tF}_{\tsigma}$; and that for every line $L\not\in \lset'_i$, its contribution to $\cro^{\tF'}_{\tsigma'}$ is at least as large as its contribution to $\cro^{\tF}_{\tsigma}$. It then follows that $\cro^{\tF'}_{\tsigma'}\geq \cro^{\tF}_{\tsigma}-O(q)$, and so
	$\WB^{F_{i+1}}_{\sigma_{i+1}}(X')\geq \WB^{F_i}_{\sigma_i}(X')-O(q)$. Therefore, in order to prove Lemma \ref{lemma: small change}, it is now enough to prove Claim \ref{claim: lines in li contribute little}.
	
\begin{proofof}{Claim \ref{claim: lines in li contribute little}}
Consider some line $L\in \lset_i'\setminus\set{L_i^*}$, and let $v\in V(T_{\tsigma})$ be the vertex to which $L$ belongs. Notice that $L$ appears in $\tsigma$ after $L_i^*$. Therefore, if $S=S(v)$ is the strip that $L$ partitioned, then at least one of the boundaries of $S$ lies in $\lset'_i$. If exactly one boundary of $S$ lies in $\lset'_i$, then we say that $S$ is an \emph{external strip}; otherwise, we say that $S$ is an internal strip. Consider now some crossing $(p,p')\in \cro_{\tsigma}(S)$. Since $L\in \lset'_i$, and at least one boundary of $S$ lies in $\lset'_i$, at least one of the points $p,p'$ must lie on a column of $\bset(C_i)$. If exactly one of $p,p'$ lie on a column of $\bset(C_i)$, then we say that $(p,p')$ is a type-1 crossing; otherwise it is a type-2 crossing. Notice that, if $S$ is an internal strip, then only type-2 crossings of $L$ are possible. We now bound the total number of type-1 and type-2 crossings separately, in the following two observations.


\begin{observation}\label{obs: type 2 crossings}
	The total number of type-2 crossings in $\bigcup_{L\in \lset_i'\setminus\set{L_i^*}}\cro_{\tsigma}(L)\leq O(q)$.
\end{observation}

\begin{proof}
	Recall that we have denoted by $X'_i$ the set of all input points that lie on the columns of $\bset(C_i)$; all type-2 crossings are between points in $X'_i$. Moreover, $X'_i$ is a monotonically increasing sequence, so from Observation \ref{obs: solution for monotone increasing set}, $\opt(X'_i)\leq |X'_i|\leq q$.
	
	Permutation $\tsigma$ of the lines in $\lset'$ naturally induces a permutation $\tsigma_i$ of the lines in $\lset'_i$. The number of type-2 crossings charged to all lines in $\lset_i'$ is then exactly $\WB_{\tsigma_i}(X'_i)$. From Claim \ref{claim: bounding WB by OPT}, $\WB_{\tsigma_i}(X'_i)\leq O(\opt(X_i))\leq O(q)$. Therefore, the total number of type-$2$ crossings in $\bigcup_{L\in \lset_i'\setminus\set{L_i^*}}\cro_{\tsigma}(L)$ is bounded by $O(q)$.	
\end{proof}


\begin{observation}\label{obs: type 2 crossings}
	The total number of type-1 crossings in $\bigcup_{L\in \lset_i'\setminus\set{L_i^*}}\cro_{\tsigma}(L)\leq O(q)$.
\end{observation}
\begin{proof}
	Consider a line $L\in \lset_i'\setminus\set{L_i^*}$, and let $S$ be the strip that it splits. Recall that, if there are any type-1 crossings in $\cro_{\tsigma}(L)$, then $S$ must be an external strip. Line $L$ partitions $S$ into two new strips, that we denote by $S'$ and $S''$. Notice that exactly one of these strips (say $S'$) is an internal strip, and the other strip is external. Therefore, the points of $X'_i\cap S'$ will never participate in type-$1$ crossings again. Recall that, from Observation \ref{obs: number of crossings at most min of both sides}, the total number of crossings in $\cro_{\tsigma}(L)$ is bounded by $2|S'\cap X'_i|$. We say that the points of $S'\cap X'_i$ pay for these crossings. Since every point of $X'_i$ will pay for a type-1 crossing at most once, we conclude that the total number of type-1 crossings in $\bigcup_{L\in \lset_i'\setminus\set{L_i^*}}\cro_{\tsigma}(L)$ is bounded by $2|X'_i|\leq 2q$.
\end{proof}

We conclude that the total number of all crossings in $\bigcup_{L\in \lset_i'\setminus\set{L_i^*}}\cro_{\tsigma}(L)$ is at most $O(q)$. Since, for every line $L$, $\cro_{\tsigma}^{\tF}(L)\subseteq \cro_{\tsigma}(L)$, we get that $\sum_{L\in \lset_i'\setminus\set{L_i^*}}|\cro^{\tF}_{\tsigma}(L)|\leq O(q)$.
\end{proofof}			
\end{proof}


To summarize, we have transformed a permutation $\sigma'$ of $\lset'$ into a permutation $\sigma''$ of $\lset'$, and we have shown that  $\WB_{\sigma''}(X')\geq \WB^F_{\sigma'}(X')-O(Nq)\geq \WB_{\sigma'}(X')/4-O(Nq)$. 


\paragraph{Transforming $\sigma''$ into $\sigma$.}
In this final step, we transform the permutation $\sigma''$ of $\lset'$ to a permutation $\sigma$ of $\lset$, and we will show that $\WB_{\sigma}(X)\geq \WB_{\sigma''}(X')-O(Nq)$.

The transformation is straightforward. Consider some column $C_i\in \cset$, and the corresponding set $\lset'_i\subseteq \lset'$ of lines.
Recall that the lines in $\lset'_i$ are indexed $L^1_i,\ldots,L^{q+1}_i$ in this left-to-right order, where $L^1_i$ appears to the left of the first column of $\bset(C_i)$,a nd $L^{q+1}_i$ appears to the right of the last column of $\bset(C_i)$. Recall also that, in the current permutation $\sigma''$, one of the following happens: either (i) line $L^1_i$ appears in the permutation first, and lines $L^{q+1}_i,L^2_i,\ldots, L^q_i$ appear at some later point consecutively in this order; or (ii) line $L^{q+1}_i$ appears in the permutation first, and lines $L^1_i,L^2_i,\ldots,L^q_i$ appear somewhere later in the permutation consecutively in this order. Therefore, for all $2\leq j\leq q$, line $L_i^j$ separates a strip whose left boundary is $L_i^{j-1}$ and right boundary is $L_i^{q+1}$. It is easy to see that the cost of each such line $L_i^j$ in permutation $\sigma''$ is at most $1$.

Let $\sigma^*$ be a sequence of lines obtained from $\sigma''$ by deleting, for all $1\leq i\leq N$, all lines $L_i^2,\ldots,L_i^q$ from it. Then $\sigma^*$ naturally defines a permutation $\sigma$ of the set $\lset$ of vertical lines. Moreover, from the above discussion, the total contribution of all deleted lines to $\WB_{\sigma''}(X')$ is at most $Nq$, so $\WB_{\sigma}(X)\geq \WB_{\sigma''}(X')-O(Nq)\geq \WB_{\sigma'}(X')/4-O(Nq)\geq \WB(X')/4-O(Nq)$. We conclude that $\WB(X)\geq \WB_{\sigma}(X)\geq \WB(X')/4-O(Nq)$.




\iffalse
\section{Upper Bound for $\WB(X^*)$}

In this section we show that $\WB(X^*)=O(N^*\log\log\log N^*)$. Recall that we have established that $\opt(X^*)=\Omega(N^*\log\log N^*)$, so 	 we obtain a gap of $\Omega(\log\log N^*/\log\log\log N^*)$ between $\opt(X^*)$ and $\WB(X^*)$.

Recall that our starting point is the instance $\hat X$, that has $N^*=N\log N$ points. Recall that we have defined a collection $\cset$ of columns that contains every column with an integral $x$ -coordinate between $1$ and $N$ inclusively; the points of $\hat X$ lie on the columns of $\cset$, with exactly $\log N$ points lying on each such column.

Recall that, in order to obtain instance $X^*$, we have replaced every column $C\in \cset$ with a collection $\bset(C)$ of $\log N$ new columns. Let $\cset'=\bigcup_{C\in \cset}\bset(C)$ be the resulting new set of columns. For each $C\in \cset$, every point of $\hat X$ that lie on $C$ is mapped to one of the columns in $\bset(C)$ (we preserve the original row of the point), so that (i) each column in $\bset(C)$ has exactly one point lying on it; and (ii) the points that lie on the columns of $\bset(C)$ form a monotonically increasing sequence.

We will analyze $\WB(X^*)$ by relating it to $\WB(\hat X)$. In order to do so, it would be convenient for us to slightly modify the instance $\hat X$ by simply multiplying all $x$-coordinates of points of $\hat X$ and of columns of $\cset$ by factor $2$. Note that this does not affect the value of the optimal solution or of the Wilber Bound; but it ensures that every consecutive pair of columns in $\cset$ is separated by a column with an integral $x$-coordinate.

Similarly, we modify the instance $X^*$, by inserting, for every consecutive pair $C,C'$ of columns of $\cset$, a new column that lies between the columns of $\bset(C)$ and the columns of $\bset(C')$. We denote by $\cset''$ the set of all columns of $X^*$ that have integral coordinates. This transformation does not affect the optimal solution cost or the value of the Wilber Bound. Let $\tilde C,\tilde C'$ be the first and the last columns of $\cset''$.

Let $\lset'$ be the set of all vertical lines with half-integral coordinates that lie between columns $\tilde C$ and $\tilde C'$. For every column $C\in \cset$ in the original instance $\hat X$, we let $L'(C),\in \lset'$ be the vertical line with a half-integral coordinate that lies immediately before the first column of $\bset(C)$, and we let $L''(C)\in \lset'$ be the vertical line with a half-integral coordinate that lies immediately after the last column of $\bset(C)$. Let $\lset'(C)$ be the set of all vertical lines with half-integral coordinates that lie between $L'(C)$ and $L''(C)$, including these two lines. Denote $\lset'(C)=(L_1(C),L_2(C),\ldots,L_{\log N+1}(C))$, where $L_1(C)=L'(C)$, $L_{\log N+1}(C)=L''(C)$, and the lines are indexed in their natural left-to-right order.
Note that $\lset'=\bigcup_{C\in \cset}\lset'(C)$.

The remainder of this section is dedicated to the proof of the following theorem.

\begin{theorem}\label{thm: WB for second final instance}
	For every permutation $\sigma'$ of $\lset'$, $\WB_{\sigma'}(X^*)=O(N^*\log\log\log N^*)$.
\end{theorem}

In order to prove the theorem, we fix a permutation $\sigma'$ of $\lset'$. We perform a slight modification of this permutation, to obtain a new permutation $\sigma''$, such that $\WB_{\sigma''}(X^*)$ is close to $\WB_{\sigma'}(X^*)$. Permutation $\sigma''$ has the property that for every column $C\in \cset$ of the original instance $\hat X$, all lines of $\lset'(C)$ (except for one) appear consecutively in $\sigma''$. It is then easy to use $\sigma''$ in order to define a permutation $\sigma$ of the set $\lset$ of all vertical lines with half-integral coordinates in instance $\hat X$. We then show that $\WB_{\sigma''}(X^*)$ is close to $\WB_{\sigma}(\hat X)$.


\subsection{Transforming the Permutation}
Let $\sigma'$ be any permutation of the set $\lset'$ of all vertical lines with half-integral $x$-coordinates for instance $X^*$. 
Consider the partitioning tree $T=T(\sigma')$ associated with $\sigma'$, and some vertex $v\in V(T)$. Let $S=S(v)$ be the vertical strip associated with $v$, and let $L\in \lset'$ be the vertical line that belongs to $v$. Let $\cro_{\sigma'}(L)$ be the set of all crossings $(p,p')$ that contribute to $\cost(L)$; that is, $p$ and $p'$ are two points that lie in $S$ on two opposite sides of $L$, and no other point of $X^*\cap S$ lies between the row of $p$ and the row of $p'$. Let $\cro_{\sigma'}=\bigcup_{L\in \lset'}\cro_{\sigma'}(L)$, so $|\cro_{\sigma'}|=\WB_{\sigma'}(X^*)$.


For our analysis, it would be convenient to modify the way we compute the Wilber Bound. Specifically, we will define a subset $F\subseteq X^*$ of input points that we call \emph{forbidden points}, and we will ignore all crossings in which the forbidden points participate. We will choose $F$ such that the total number of the remaining crossings is large enough. We will then restrict the Wilber Bound to only counting crossings that do not involve the forbidden points. This will help us in relating the Wilber Bound of the two permutations.

We now describe the procedure for defining the forbidden points. The input to the procedure is some permutation $\sigma'$ of the set $\lset'$ of lines.
We consider every column $C\in \cset$ of the original instance $\hat X$ one-by-one. Consider now any such column $C\in \cset$. Let $L(C)$ be the first line of $\lset(C)$ that appears in the permutation $\sigma'$. We select a random bit $b(C)\in \set{0,1}$ with probability $1/2$, independently from all other choices. If $b(C)=0$, then we say that every point of $X^*$ that lies on a column of $\bset(C)$ to the left of $L$ is a \emph{forbidden point}; otherwise, we say that every point of $X^*$ that lies on a column of $\bset(C)$ to the right of $L$ is a forbidden point.  

Assume now that we are given an arbitrary set $F$ of forbidden points of $X^*$ (which may or may not have been defined using the above procedure). For a permutation $\sigma'$ of $\lset'$, we let $\cro^F_{\sigma'}\subseteq \cro_{\sigma'}$ contain only those crossings $(p,p')$ for which neither $p$ nor $p'$ are forbidden points. We can now define the Wilber Bound with respect to $F$ to be $\WB_{\sigma'}^F(X^*)=\cro^F_{\sigma'}$.


We now assume that the permutation $\sigma'$ is fixed, and we run the above algorithm to select the bits $b(C)$ for all $C\in \cset$ and to define the set $F$ of forbidden points.  It is easy to verify, that, for every crossing $(p,p')\in \cro_{\sigma'}$, with probability at least $1/4$, the crossing is not discarded. Therefore, there is a choice of the bits $b(C)\in \set{0,1}$ for $C\in \cset$, such that, if $F$ is the resulting set of forbidden points, then $\WB^F_{\sigma'}(X^*)\geq \WB_{\sigma'}(X^*)/4$. 


We now show how to transform $\sigma'$ into a new permutation $\sigma''$. We will then show that $WB^F_{\sigma''}(X^*)$ is large compared to $\WB_{\sigma'}^F(X^*)$ (the set $F$ of forbidden points remains unchanged, and was defined with respect to $\sigma'$).
We perform the transformation gradually, by considering every column $C\in \cset$ of the original instance $\hat X$ one-by-one. For each such column $C\in \cset$, we transform $\sigma'$, as follows. 
If $b(C)=0$, we start by switching the locations of $L(C)$ and $L'(C)$ -- the left-most line of $\lset(C)$. Therefore, $L'(C)$ is now the first line of $\bset(C)$ that appears in $\sigma'$. Next, we let $\hat L(C)$ be the last line of $\bset(C)$ in the permutation. We move the lines $L_2(C),\ldots,L_{\log N+1}(C)$ to appear at the location of $\hat L(C)$ in the permutation, in this order.

If $b(C)=1$, then we start by switching the locations of $L(C)$ and $L''(C)$ --  the right-most line of $\lset(C)$. We then move $L_{\log N+1}(C), L_2(C),L_3(C),\ldots,L_{\log N}(C)$ to appear at the location of $\hat L(C)$ in the permutation, in this order.


Once we process every column $C\in \cset$, we obtain the final permutation $\sigma''$ of $\lset'$. The following lemma is central to our analysis.

\begin{lemma}\label{lemma: small change}
	For every column $C\in \cset$, if we denote by $\sigma_1$ the permutation $\sigma'$ before column $C$ was processed, and by $\sigma_2$ the permutation $\sigma'$ after column $C$ was processed, then $\WB^F_{\sigma_2}(X^*)\geq \WB^F_{\sigma_1}(X^*)-O(\log N)$.
\end{lemma}

\begin{proof}
	Consider a line $L\in \lset'$. Recall that $\cro_{\sigma_1}(L)$ is the set of all crossings that are charged to the line $L$ in permutation $\sigma_1$. We let $\cro^F_{\sigma_1}(L)\subseteq \cro_{\sigma_1}(L)$ be obtained from the set  $\cro_{\sigma_1}(L)$ of crossings, by discarding all crossings $(p,p')$ where $p\in F$ or $p'\in F$ holds. We define $\cro^F_{\sigma_2}(L)$ similarly.
	
	We start by showing that for every line $L\in \lset'$ that does not lie in $\lset(C)$, $\cro^F_{\sigma_1}(L)=\cro^F_{\sigma_2}(L)$
	
	\begin{claim}\label{claim: lines outside of block do not change}
		For every line $L\in \lset'\setminus \lset(C)$, $|\cro^F_{\sigma_2}(L)|\geq |\cro^F_{\sigma_1}(L)|$.
	\end{claim}
\begin{proof}
	Consider any line $L\in \lset'\setminus \lset(C)$. Let $v\in V(T_{\sigma_1})$ be the vertex to which $L$ belongs, and let $S=S(v)$ be the corresponding strip. Similarly, we define $v'\in V(T_{\sigma_2})$ and $S'=S(v')$ with respect to $\sigma_2$. Let 
	 Recall that $L(C)$ is the first line of $\lset(C)$ that appears in $\sigma'$ (and hence in $\sigma_1$), and $\hat L(C)$ is the last such line. We now consider five cases.
	
	
	First, if $L$ appears before $L(C)$ in $\sigma_1$, then the prefixes of the sequences $\sigma_1$ and $\sigma_2$ until the appearance of the line $L(C)$ are identical, so $S=S'$, and $|\cro^F_{\sigma_1}(L)|=|\cro^F_{\sigma_2}(L)|$.
	
	Second, if $L$ appears after $\hat L(C)$ in $\sigma_1$, then, if we denote by $\tilde \lset\subseteq \lset'$ the set of all lines that lie before $L$ in $\sigma_1$, and define $\tilde \lset'$ similarly for $\sigma_2$, then $\tilde \lset=\tilde \lset_2$. Therefore, the strip $S$ that line $L$ partitions is the same in both cases, and so $S=S'$, and $|\cro^F_{\sigma_1}(L)|=|\cro^F_{\sigma_2}(L)|$.
	
	The third case is when $L$ appears between $L(C)$ and $\hat L(C)$ in $\sigma_1$, but neither boundary of the strip $S$ belongs to $\lset(C)$. It is then easy to verify that $S=S'$, and $|\cro^F_{\sigma_1}(L)|=|\cro^F_{\sigma_2}(L)|$.
	
	The fourth case is when $L$  appears between $L(C)$ and $\hat L(C)$ in the permutation $\sigma_1$, and the left boundary of $S$ belongs to $\lset(C)$.
	
	If $b(C)=0$, then we have replaced $L(C)$ with the line $L'(C)$, that lies to the left of $L(C)$. Therefore, the right boundary of $S$ remains the same, and the left boundary is pushed to the left. This can only increase the set of crossings that are charged to $L$, so $|\cro^F_{\sigma_1}(L)|\geq |\cro^F_{\sigma_2}(L)|$.
	
	If $b(C)=1$, then we have replaced $L(C)$ with the line $L''(C)$, that lies to the right of $L(C)$. If $(p,p')\in \cro_{\sigma_1}(L)$, where one of the points lies to the left of $L''(C)$, then this crossing no longer belongs to $\cro_{\sigma_2}(L)$. However, we claim that each such crossing involves a forbidden vertex, and cannot be counted in $\cro^F_{\sigma_1}(L)$. Indeed, let $(p,p')\in \cro_{\sigma_1}(L)$ be any crossing, and assume w.l.o.g. that $p$ lies to the left of $L''(C)$. Recall that, since $b(C)=1$, all points that lie between $L(C)$ and $L''(C)$ are forbidden. Therefore, it is enough to show that $p$ lies to the right of $L(C)$. Recall that we have assumed that $L$ appears after $L(C)$ in the permutation $\sigma_1$. Therefore, the left boundary of $S$ must either coincide with $L(C)$ or lie to the right of it. Therefore, $p$ lies to the right of $L(C)$, and it is a forbidden point.
	
	The fifth case, when $L$ appears between $L(C)$ and $\hat L(C)$ in the permutation $\sigma_1$, and the right boundary of $S$ belongs to $\lset(C)$ is symmetric to the fourth case.	
\end{proof}

It now remains to analyze the crossings of the lines in $\lset(C)$. We do so in the following two claims. The first claim shows that switching $L(C)$ with $L'(C)$ or $L''(C)$ does not decrease the number of crossings.

\begin{claim}
 If $b=0$, then	$|\cro^F_{\sigma_2}(L'(C))|\geq |\cro^F_{\sigma_1}(L(C))|$; if $b=1$, then $|\cro^F_{\sigma_2}(L''(C))|\geq |\cro^F_{\sigma_1}(L(C))|$.
\end{claim}

\begin{proof}
	
\end{proof}



	
\end{proof}






Notice that, if the lemma is true, then $\WB_{\sigma''}(X^*)\geq WB_{\sigma'}(X^*)-O(|\cset|\cdot \log N)\geq WB_{\sigma'}(X^*)-O(N\log N)\geq WB_{\sigma'}(X^*)-O(N^*)$.

\fi


==> test.tex <==
Hello

